SLATE: Are AI-Generated Slides Educationally Effective? A Benchmark for Language Teaching Quality and Learner Knowledge Acquisition

LLMs have achieved remarkable capabilities in generating language teaching slides. However, a critical mismatch persists between visual polish and actual instructional effectiveness. To address this gap, we introduce SLATE (Slide-based Learning Assessment for Teaching Effectiveness), the first benchmark that evaluates AI-generated language teaching slides through instructional effectiveness and learner knowledge acquisition. SLATE transforms linguistics olympiad puzzles from low-resource languages with negligible web presence into 90 standardized instructional units comprising 1,133 assessable items, paired with a structured course outline and matched near- and far-transfer test sets. This pretest-posttest design eliminates pretrained knowledge leakage, ensuring gains reflect learning rather than prior recall. Using VLMs as scalable learner proxies and directionally supported by a three-system human pilot, our results show that content validity exhibits a weak association with learning gain, while pedagogical design exhibits a robust positive association. Moreover, most systems show a significant gap between near- and far-transfer accuracy, and even frontier models can produce negative learning gains. SLATE reveals a dissociation between artifact quality and instructional effectiveness, calling for a paradigm shift in how generative teaching systems are built, evaluated, and deployed.

==> tables/exp_d3_table.tex <==
\begin{table*}[!t]
\small
\centering
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{l|ccccc|cc}
\toprule
\multirow{2}*{\makecell*[l]{System}} 
& \multicolumn{5}{c|}{\makecell*[c]{Deck Statistics}}
& \multicolumn{2}{c}{\makecell*[c]{Instruction-Supportive Visuals}} \\
& Slides & WPS & Tables & Colors & VA (\%) & Exercise (\%) & Note \\
\midrule
Claude Opus 4.7 & \textbf{13.2} & 72.6 & \textbf{7.0} & 17.0 & \textbf{99} & \textbf{100} & balanced, table-rich \\
Qwen3.6-Max & 12.3 & 76.5 & 4.9 & 19.9 & \textbf{99} & 99 & high VA, compact \\
GPT-5.4 & 12.3 & 72.1 & 6.7 & 16.3 & \textbf{99} & \textbf{100} & strong structure \\
MiniMax-M2.7 & 12.0 & 83.5 & 6.7 & 25.8 & \textbf{99} & \textbf{100} & colorful, dense \\
Qwen3.6-Plus & 11.6 & 71.4 & 4.4 & 17.5 & \textbf{99} & \textbf{100} & efficient layout \\
Kimi-K2.6 & 11.1 & 60.3 & 3.9 & 19.4 & 91 & 90 & lighter content \\
GLM-5.1 & 8.9 & \textbf{103.3} & 4.3 & 18.9 & 80 & 78 & text-heavy \\
Gemini-3.1-Pro & 7.3 & 60.4 & 2.5 & 12.9 & 79 & 70 & sparse support \\
Claude Sonnet 4.6 & 6.0 & 95.4 & 3.2 & \textbf{36.7} & 98 & 96 & visually strong, shorter \\
DeepSeek-V4-Pro & 3.6 & 73.3 & 1.1 & 15.6 & 61 & 78 & insufficient deck length \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{D3-related deck statistics and visual support indicators.} WPS denotes average words per slide. VA is the visual-aid coverage score. Exercise is the proportion of decks that contain explicit practice or interactive elements.}
\label{tab:exp-d3-results}
\end{table*}


==> tables/exp_main_table.tex <==
\begin{table*}[!t]
\small
\centering
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{l|cc|cc|cc|c}
\toprule
\multirow{2}*{\makecell*[l]{System}} 
& \multicolumn{2}{c|}{\makecell*[c]{Content \& Pedagogy}}
& \multicolumn{2}{c|}{\makecell*[c]{Visual Design}}
& \multicolumn{2}{c|}{\makecell*[c]{Learning \& Transfer}}
& \multirow{2}*{\makecell*[c]{AVG}} \\
& D1 & D2 & VA (\%) & Exercise (\%) & Gain & Post-test & \\
\midrule
\rowcolor{gray!12}
\multicolumn{8}{c}{\textit{Closed-source / Proprietary Systems}}\\
\cmidrule{1-8}
Claude Opus 4.7 & \underline{4.19} & \textbf{4.42} & \textbf{99} & \textbf{100} & \textbf{+5.46} & \textbf{29.25} & \textbf{23.72} \\
Claude Sonnet 4.6 & 4.05 & 3.96 & 98 & 96 & +1.85 & 25.63 & 21.91 \\
GPT-5.4 & \textbf{4.23} & \underline{4.28} & \textbf{99} & \textbf{100} & +2.61 & 26.40 & \underline{22.90} \\
DeepSeek-V4-Pro & 3.61 & 3.54 & 61 & 78 & -1.68 & 22.10 & 15.71 \\
Qwen3.6-Plus & 4.07 & 4.16 & \textbf{99} & \textbf{100} & +0.38 & 24.17 & 21.36 \\
Kimi-K2.6 & 4.07 & 4.18 & 91 & 90 & -0.89 & 22.90 & 20.25 \\
GLM-5.1 & 3.88 & 4.01 & 80 & 78 & -1.24 & 22.54 & 19.61 \\
MiniMax-M2.7 & 3.96 & 4.12 & \textbf{99} & \textbf{100} & +3.27 & 27.06 & 22.60 \\
Gemini-3.1-Pro & 3.75 & 3.82 & 79 & 70 & -2.51 & 21.28 & 17.48 \\
Qwen3.6-Max & -- & -- & \textbf{99} & 99 & \underline{+5.14} & \underline{28.92} & -- \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Main results on SLATE} across artifact-level and learner-level dimensions.} AVG is the arithmetic mean of the six visible columns after linearly rescaling VA and Exercise to the same 0--100 range as reference context for comparison; it is intended only as a compact summary. Within the currently available systems, the best result in each column is \textbf{bolded} and the second-best is \underline{underlined}. D1/D2 values for Qwen3.6-Max are pending expert/model scoring and are therefore left blank.}
\label{tab:exp-main-results}
\end{table*}


==> tables/main_results.tex <==
\begin{table*}[!t]
\small
\centering
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l|cc|ccc|c}
\toprule
\multirow{2}*{\makecell*[l]{System / Setting}} 
& \multicolumn{2}{c|}{\makecell*[c]{Artifact Quality}}
& \multicolumn{3}{c|}{\makecell*[c]{Learning \& Transfer}}
& \multirow{2}*{\makecell*[c]{Status}} \\
& D1 $\uparrow$ & D2 $\uparrow$ & Post-test $\uparrow$ & Near $\uparrow$ & Far $\uparrow$ & \\
\midrule
\rowcolor{gray!12}
\multicolumn{7}{c}{\textit{Current Available Results}}\\
\cmidrule{1-7}
Main system (5-run average) & 4.19 & 4.42 & \textbf{28.0} & \textbf{25.56} & \textbf{6.67} & complete \\
\texttt{Qwen3.6-Max} & -- & -- & \textit{pending} & \textit{pending} & \textit{pending} & running \\
\bottomrule
\end{tabular}
\caption{\textbf{Main results on SLATE.} D1 and D2 are averaged over 89 evaluable cases because one item (P13) received a judge refusal. D4 values in the current main setting are reported from the stabilized experimental configuration, while the pilot-stage baseline is discussed separately in Table~\ref{tab:ablation}. We keep \texttt{Qwen3.6-Max} as a placeholder because the corresponding runs are not yet complete.}
\label{tab:main_results}
\end{table*}

